DMPCN: Dynamic Modulated Predictive Coding Network with Hybrid Feedback Representations

Traditional predictive coding networks, inspired by theories of brain function, consistently achieve promising results across various domains, extending their influence into the field of computer vision. However, the performance of the predictive coding networks is limited by their error feedback mechanism, which traditionally employs either local or global recurrent updates, leading to suboptimal performance in processing both local and broader details simultaneously. In addition, traditional predictive coding networks face difficulties in dynamically adjusting to the complexity and context of varying input data, which is crucial for achieving high levels of performance in diverse scenarios. Furthermore, there is a gap in the development and application of specific loss functions that could more effectively guide the model towards optimal performance. To deal with these issues, this paper introduces a hybrid prediction error feedback mechanism with dynamic modulation for deep predictive coding networks by effectively combining global contexts and local details while adjusting feedback based on input complexity. Additionally, we present a loss function tailored to this framework to improve accuracy by focusing on precise prediction error minimization. Experimental results demonstrate the superiority of our model over other approaches, showcasing faster convergence and higher predictive accuracy in CIFAR-10, CIFAR-100, MNIST, and FashionMNIST datasets.

==> tables/mlpreamble.tex <==
% Operators, basic concepts
\newcommand{\argmax}{\mathop{\mathrm{argmax}}\limits}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}\limits}
\newcommand{\rank}[1]{\mathsf{rank}\left(#1\right)}		% matrix rank
\newcommand{\norm}[1]{\left\|#1\right\|}				% vector/matrix norm
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\Span}[1]{\mathsf{span}\left\{#1\right\}}	% space spanned by vectors
\renewcommand{\dim}[1]{\mathsf{dim}\left(#1\right)}		% dimension of a space
\newcommand{\ran}[1]{\mathsf{ran}\left(#1\right)}		% range of a matrix
\newcommand{\Null}[1]{\mathsf{null}\left(#1\right)}		% null space of a matrix

% Vector Matrix Set Function
\newcommand{\V}[1]{\ensuremath{\bm{#1}}}
\newcommand{\M}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\Set}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\Space}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\F}[1]{\ensuremath{\mathrm{#1}}}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et~al}\onedot}
\newcommand*{\myfnsymbolsingle}[1]{%
  \ensuremath{%
    \ifcase#1% 0
    \or % 1
      *%   
    \or % 2
      \dagger
    \or % 3  
      \ddagger
    \or % 4   
      \mathsection
    \or % 5
      \mathparagraph
    \else % >= 6
      \@ctrerr  
    \fi
  }%   
}   
\makeatother
\newcommand{\Tref}[1]{Table~\ref{#1}}
\newcommand{\Eref}[1]{Equation~(\ref{#1})}
\newcommand{\Fref}[1]{Figure~\ref{#1}}
\newcommand{\Sref}[1]{Section~\ref{#1}}
\newcommand{\Aref}[1]{Algorithm~\ref{#1}}
\newcommand{\tref}[1]{Tab.~\ref{#1}}
\newcommand{\eref}[1]{Eq.~(\ref{#1})}
\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\sref}[1]{Sec.~\ref{#1}}
\newcommand{\aref}[1]{Algo.~\ref{#1}}

\newcommand*{\myfnsymbol}[1]{%
  \myfnsymbolsingle{\value{#1}}%
}

% remove upper boundary by multiplying the symbols if needed
\usepackage{alphalph}
\newalphalph{\myfnsymbolmult}[mult]{\myfnsymbolsingle}{}

\renewcommand*{\thefootnote}{%
  \myfnsymbolmult{\value{footnote}}%
}

\renewcommand*{\thempfootnote}{%
  \myfnsymbolmult{\value{mpfootnote}}%
}


==> tables/table.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we introduce a novel enhancement for traditional predictive coding networks through a hybrid prediction error feedback mechanism with dynamic modulation, effectively combining global and local contexts and adjusting feedback based on input complexity. Our approach, complemented by a specialized loss function designed for precise prediction error minimization, demonstrates superior predictive accuracy and faster convergence on benchmark datasets compared to existing methods. This work not only addresses key limitations in processing detailed and broader aspects of data and in adapting to varied input scenarios but also opens new avenues for future research in artificial intelligence and machine learning with a promising direction.
